Twisted automorphisms of Hopf algebras

Twisted homomorphisms of bialgebras are bialgebra homomorphisms from the first into Drinfeld twistings of the second. They possess a composition operation extending composition of bialgebra homomorphisms. Gauge transformations of twists, compatible with adjacent homomorphisms, give rise to gauge transformation of twisted homomorphisms, which behave nicely with respect to compositions. Here we study (gauge classes of) twisted automorphisms of cocommutative Hopf algebras. After revising well-known relations between twists, twisted forms of bialgebras and $R$-matrices (for commutative bialgebras) we describe twisted automorphisms of universal enveloping algebras.

==> xygar.tex <==
%% xygar.tex from $Id: xygar.doc,v 0.2 2002/05/20 00:00:00 steffen Exp $ -*-TeX-*-
%%
%% Xy-pic ``Generalized Arrow'' feature.
%% Copyright (c) 2000-2002 Daniel Steffen <steffen@ics.mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1996 Kristoffer H. Rose <krisrose@brics.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this macro package; if not, write to the Free Software Foundation,
%% Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
%%
\ifx\xyloaded\undefined \input xy \fi

\xyprovide{gar}{Generalized Arrow feature}{\stripRCS$Revision: 0.2 $}%
 {Daniel A. Steffen}{steffen@ics.mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}

\message{generalized arrow,}
\xyrequire{curve}\xyrequire{arrow}\xycatcodes
\xydef@\gardefaultlength#1{\A@=#1\relax \divide\A@ 2%
\edef\gardefaulthlen@@{\expandafter\the\A@}}

\xydef@\gardefaultform#1{\def\gardefaultform@@{#1}}

\gdef\glabel#1{\save\POS="garlabel@#1"\restore}
\gdef\glabelar#1{\save\POS?="garlabel@#1"\restore}

\gardefaultform{\addAT@\string2}
\gardefaultlength{1em}

\xylet@\garsrc@@=\empty
\xylet@\gartgt@@=\empty
\xylet@\garvariant@@=\empty
\xylet@\garcurve@@=\empty
\xylet@\garpos@@=\empty
\xylet@\garhlen@@=\empty
\xylet@\garlabels@@=\empty

\xydef@\gar{\relax\garSAFE}
\xydef@\garSAFE{%
\def\garsrc@@{nosrc}%
\def\gartgt@@{notgt}%
\edef\garvariant@@{}%
\edef\garcurve@@{}%
\edef\garpos@@{.5}%
\edef\garhlen@@{\gardefaulthlen@@}%
\def\garlabels@@{}%
\xyFN@\gar@}

\xydef@\gar@{%
\ifx \space@\next \expandafter\DN@\space{\xyFN@\gar@}%
\else \addAT@\ifx\next \DN@{\garvariant@}%
\else\ifx [\next \DN@ [##1,##2]{\garsrctgt@{##1}{##2}}%
\else \let\next@=\gar@error \fi\fi\fi \next@}

\xydef@\gar@error#1{\xyerror@{Illegal gar (\meaning\next)}{}\xyFN@\gar@}

\xydef@\gar@@{%
\ifx \space@\next \expandafter\DN@\space{\xyFN@\gar@@}%
\else\ifx (\next \DN@ (##1){\garpos@{##1}}%
\else\addLT@\ifx\next \addGT@{\addLT@\DN@##1}{\garlen@{##1}}%
\else\ifx |\next \DN@ |##1{\gar@anchor{|{##1}}}%
\else\ifx ^\next \DN@ ^##1{\gar@anchor{^{##1}}}%
\else\ifx _\next \DN@ _##1{\gar@anchor{_{##1}}}%
\else \let\next@=\gar@x \fi\fi\fi\fi\fi\fi \next@}

\xydef@\garsrctgt@#1#2{%
\def\garsrc@@{#1}%
\def\gartgt@@{#2}%
\xyFN@\gar@@}

\xydef@\garvariant@{%
\ifx \space@\next \DN@{\xyFN@\gar@}%
\else \addAT@\ifx\next \DN@##1{\addAT@\addtogarvariant@\xyFN@\garvariant@}%
\else \ifx [\next \DN@{\xyFN@\gar@}%
\else \ifx \bgroup\next \DN@##1{\addtogarvariant@{{##1}}\xyFN@\garvariant@}%
\else \ifx /\next \DN@ /##1/{\garcurve@{##1}}%
\else \DN@##1{\addtogarvariant@{##1}\xyFN@\garvariant@}%
\fi\fi\fi\fi\fi \next@}

\xydef@\addtogarvariant@#1{%
\expandafter\def\expandafter\garvariant@@\expandafter{\garvariant@@#1}}

\xydef@\garcurve@#1{%
\def\garcurve@@{#1}%
\addLQ@\addtogarvariant@%
\addtogarvariant@{{{?}}}%
\xyFN@\garvariant@}

\xydef@\garpos@#1{%
\def\garpos@@{#1}%
\xyFN@\gar@@}

\xydef@\garlen@#1{%
\A@=#1\relax \divide\A@ 2%
\edef\garhlen@@{\expandafter\the\A@}%
\xyFN@\gar@@}

\xydef@\gar@anchor#1{%
\expandafter\def\expandafter\garlabels@@\expandafter{\garlabels@@ #1}%
\xyFN@\gar@@}

{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{
\save"garlabel@#1";"garlabel@#2"**\crv{~*={}{**{} ? +/#6/+/#6/}}
\ar#5#7?(#3)/-#4/;?(#3)/#4/
\restore}}
\xylet@\g@rc=\next

{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{
\save"garlabel@#1";"garlabel@#2"**{}
\ar#5#7?(#3)/-#4/;?(#3)/#4/
\restore}}
\xylet@\g@r=\next

\xydef@\gar@x{%
\ifx\garvariant@@\empty\edef\garvariant@@{\gardefaultform@@}\fi%
\ifx\garcurve@@\empty \addtotoks@{\g@r}%
\else \addtotoks@{\g@rc}\fi%
\expandafter\addtotoks@\expandafter{\expandafter{\garsrc@@}}%
\expandafter\addtotoks@\expandafter{\expandafter{\gartgt@@}}%
\expandafter\addtotoks@\expandafter{\expandafter{\garpos@@}}%
\expandafter\addtotoks@\expandafter{\expandafter{\garhlen@@}}%
\expandafter\addtotoks@\expandafter{\expandafter{\garvariant@@}}%
\expandafter\addtotoks@\expandafter{\expandafter{\garcurve@@}}%
\expandafter\addtotoks@\expandafter{\expandafter{\garlabels@@}}%
\expandafter\DNii@\expandafter{\the\toks@}\toks@={}%
\nextii@}
\xyendinput


